Fermi liquids and non--Fermi liquids

Contents I. Introduction II. Fermi Liquids III. Renormalization group for interacting fermions IV. Luttinger liquids V. Transport in a Luttinger liquid VI. The Bethe ansatz: a pedestrian introduction VII. Conclusion and outlook

==> houchesa.tex <==
%auto-ignore

\appendix
\section{Correlation functions of the Luttinger model}

\section{Coulomb gas analogy of $g_{1\perp}$}

perturbation expansion of partiton function
\begin{eqnarray*}
Z & = & Z_0 \; \Delta Z \\
\Delta Z & = & \sum_{n=0}^{\infty} \frac{1}{(2n)!}
\left[ \frac{2g_{1\perp}}{(2\pi\alpha)^2} \right]^{2n}
\prod_{\nu =1}^{2n} \int_0^L dx_\nu \int_0^\beta d\tau_\nu \\
 \times & \lefteqn{\langle T_\tau [\cos (\sqrt8 \phi_\sigma(x_1\tau_1))\dots
\cos (\sqrt8 \phi_\sigma(x_{2n}\tau_{2n}))]\rangle} &
\end{eqnarray*}
calculate correlation functions $\Rightarrow$ \\
partition function of two--component plasma
\begin{equation}
\Delta Z = \sum_{n=0}^\infty \frac{e^{2n\beta_g \mu}}{(n!)^2}
\int \prod_{\nu=1}^{2n} \frac{d^2r_\nu}{\alpha^2}
\exp(\beta_g \sum_{i<j} s_i s_j \ln|\vec{r_i} - \vec{r_j}|  )
\end{equation}
{\small $s_1 \dots s_n = 1 , s_{n+1}\dots s_{2n}= -1 \leftrightarrow
\exp(\pm i\sqrt8 \phi_\sigma)$
\\ eff. temperature: $\beta_g = 4K_\sigma$, chem. pot.: $e^{\beta_g\mu}
=\frac{g_{1\perp}}{4\pi^2 u_\sigma}$}

Perturbative calculation for small $g_{1\perp}$ ($\Leftrightarrow$
screening):
\begin{equation}
K_\sigma^{\mbox{\it eff}} = K_\sigma - \frac{g_{1\perp}^2}{2 \pi^2
u_\sigma^2} K_\sigma^2
\int_\alpha^\infty \frac{dr}{\alpha} \left(\frac{r}{\alpha}\right)
^{3-4K_\sigma} \end{equation}
change $\alpha \rightarrow \alpha e^\ell$ $\Rightarrow$ renormalization
equation
\begin{equation}\frac{d g_1(\ell)}{d \ell} = - \frac{g_1(\ell )^2}{\pi v_F} \end{equation}

